Cost-Effective Retraining of Machine Learning Models

It is important to retrain a machine learning (ML) model in order to maintain its performance as the data changes over time. However, this can be costly as it usually requires processing the entire dataset again. This creates a trade-off between retraining too frequently, which leads to unnecessary computing costs, and not retraining often enough, which results in stale and inaccurate ML models. To address this challenge, we propose ML systems that make automated and cost-effective decisions about when to retrain an ML model. We aim to optimize the trade-off by considering the costs associated with each decision. Our research focuses on determining whether to retrain or keep an existing ML model based on various factors, including the data, the model, and the predictive queries answered by the model. Our main contribution is a Cost-Aware Retraining Algorithm called Cara, which optimizes the trade-off over streams of data and queries. To evaluate the performance of Cara, we analyzed synthetic datasets and demonstrated that Cara can adapt to different data drifts and retraining costs while performing similarly to an optimal retrospective algorithm. We also conducted experiments with real-world datasets and showed that Cara achieves better accuracy than drift detection baselines while making fewer retraining decisions, ultimately resulting in lower total costs.

==> algo.tex <==
\begin{algorithm}[tb]
    \caption{\algo Algorithm}
    \label{alg:algo-template}
 \begin{algorithmic}
    \STATE {\bfseries Input:} Data \Dt, Queries \Qt, Model \model
    \STATE {\bfseries Output:} Strategy \strategy
    \STATE Compute cost matrix \costmatrix with offline data
    \STATE $\algoparamsopt  = \textsc{OfflineOptimize}(\costmatrix,\algoparams)$
    \STATE Start online evaluation with $\tprime=\T_{\offline}+1$ 
    \STATE $\strategy = \emptyset$
    \STATE Train model \Mtprime
    \FOR{$i=\T_\offline+1$ {\bfseries to} $\T$}
        \STATE $result = \decision(\ttime,\tprime,\algoparamsopt)$
        \IF{$result = \text{Retrain}$}
            \STATE $\tprime = i$ and retrain \Mtprime
        \ENDIF 
        \STATE $\strategy = \strategy \cup \braces{\tprime}$
    \ENDFOR
    \STATE {\bf Return } \strategy
 \end{algorithmic}
 \end{algorithm}

==> macros.tex <==
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{booktabs} % for professional tables
% algorithms
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{subcaption}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage[show]{chato-notes}
\usepackage[normal]{threeparttable}
\usepackage{hyperref}
\usepackage{setspace}
% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}
\usepackage[capitalize,noabbrev]{cleveref}
\RequirePackage{algorithm}
\RequirePackage{algorithmic}
\makeatletter
\newcommand\thefontsize{The current font size is: \f@size pt}
\makeatother


\newcommand{\bigObound}{\ensuremath{\mathcal{O}}}
\newcommand*{\alert}[1]{\textcolor{red}{#1}}
\newcommand{\revision}[1]{{\color{black}#1}}
\newtheorem{problem}{Problem}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand*{\R}{\mathbb{R}}
\newcommand*{\E}{\mathbb{E}}

\newcommand{\para}[1]{\noindent\textbf{#1}}
\newcommand{\spara}[1]{\smallskip\noindent\textbf{#1}}

\newcommand{\norm}[1]{\|#1\|}
\newcommand{\inner}[2]{\langle #1, #2 \rangle}
\newcommand{\round}[1]{\left(#1\right)}
\newcommand{\braces}[1]{\left\{#1\right\}}
\newcommand{\squares}[1]{\left[#1\right]}
\newcommand{\product}[1]{\left\langle#1\right\rangle}

\newcommand*{\ml}{ML}

\newcommand*{\decision}{\ensuremath{\mathcal{R}}\xspace}
% \newcommand*{\QDM}{\ensuremath{\text{\sc QDM}}\xspace}
\newcommand*{\QDMq}{\ensuremath{\psi}\xspace}
\newcommand*{\QDM}{\ensuremath{\Psi}\xspace}
% \newcommand*{\QDMdiff}{\ensuremath{\QDM_{\text{diff}}}\xspace}
\newcommand*{\QDMdiff}{\ensuremath{\overline{\Psi}}\xspace}
\newcommand*{\simfn}{\ensuremath{\text{sim}}\xspace}
\newcommand*{\loss}{\ensuremath{\ell}\xspace}
\newcommand*{\tprime}{\ensuremath{t^{\prime}}\xspace}
\newcommand*{\feat}{\ensuremath{d}\xspace}
\newcommand*{\q}{\ensuremath{q}\xspace}
\newcommand*{\x}{\ensuremath{x}\xspace}
\newcommand*{\y}{\ensuremath{y}\xspace}
\newcommand*{\X}{\ensuremath{\mathbf{X}}\xspace}
\newcommand*{\Y}{\ensuremath{\mathbf{y}}\xspace}
\newcommand*{\Yset}{\ensuremath{\mathcal{Y}}\xspace}
\newcommand*{\Xset}{\ensuremath{\mathcal{X}}\xspace}
\newcommand*{\ttime}{\ensuremath{t}\xspace}
\newcommand*{\data}{\ensuremath{D}\xspace}
\newcommand*{\model}{\ensuremath{M}\xspace}
\newcommand*{\query}{\ensuremath{Q}\xspace}
\newcommand*{\Dtprime}{\ensuremath{\data_{\tprime}}\xspace}
\newcommand*{\Mtprime}{\ensuremath{\model_{\tprime}}\xspace}
\newcommand*{\Qtprime}{\ensuremath{\query_{\tprime}}\xspace}
\newcommand*{\Dt}{\ensuremath{\data_{t}}\xspace}
\newcommand*{\Mt}{\ensuremath{\model_{t}}\xspace}
\newcommand*{\Qt}{\ensuremath{\query_{t}}\xspace}
\newcommand*{\dataBatch}{\ensuremath{B_\data}\xspace}
\newcommand*{\queryBatch}{\ensuremath{B_\query}\xspace}
\newcommand*{\T}{\ensuremath{T}\xspace}
\newcommand*{\offline}{\text{offline}\xspace}
\newcommand*{\online}{\text{online}\xspace}
\newcommand*{\Toffline}{\ensuremath{\T_{\offline}}\xspace}
\newcommand*{\Tonline}{\ensuremath{\T_{\online}}\xspace}
\newcommand*{\Tstart}{\ensuremath{\T_{\text{start}}}\xspace}
\newcommand*{\Tend}{\ensuremath{\T_{\text{end}}}\xspace}
\newcommand*{\Cost}{\ensuremath{C}\xspace}
\newcommand*{\totalcost}{\ensuremath{c}\xspace}
\newcommand*{\cost}[1]{\ensuremath{\text{cost}\round{#1}}\xspace}
\newcommand*{\dpcost}[2][]{%
    \ifx\\#1\\%
        \ensuremath{v\round{#2}}\xspace%
        \else%
        \ensuremath{v^{#1}\round{#2}}\xspace%
    \fi%
}
\newcommand*{\prev}{\ensuremath{p}\xspace}
\newcommand*{\dptable}{\ensuremath{V}\xspace}
\newcommand*{\costmatrix}{\Cost}
\newcommand*{\costentry}[1]{\ensuremath{c_{#1}}\xspace}
\newcommand*{\strategy}{\ensuremath{S}\xspace}
\newcommand*{\partialstrategy}{\ensuremath{\bar{\strategy}}\xspace}
\newcommand*{\partialstrategyopt}{\ensuremath{\round{\partialstrategy}^{*}}\xspace}

\newcommand*{\oracleretrains}{\ensuremath{O}\xspace}
\newcommand*{\retraincost}{\ensuremath{\kappa}\xspace}

\newcommand*{\retrain}{\texttt{Retrain}\xspace}
\newcommand*{\keep}{\texttt{Keep}\xspace}


%algorithms

\newcommand*{\oracle}{\textsc{Oracle}\xspace}
\newcommand*{\neverretrain}{\textsc{NR}\xspace}
\newcommand*{\algo}{\textsc{Cara}\xspace}
\newcommand*{\cara}{\algo}
\newcommand*{\algoparams}{\ensuremath{\theta}\xspace}
\newcommand*{\algoparamsopt}{\ensuremath{\algoparams^{*}}\xspace}

\newcommand*{\markov}{\textsc{Markov}\xspace}
\newcommand*{\algoMarkov}{\textsc{\algo-M}\xspace}
\newcommand*{\algoThresh}{\textsc{\algo-T}\xspace}
\newcommand*{\thresh}{\ensuremath{\tau}\xspace}
\newcommand*{\threshopt}{\ensuremath{\thresh^{*}}\xspace}
\newcommand*{\cumthresh}{\ensuremath{\tau_\text{cum}}\xspace}
\newcommand*{\cumthreshopt}{\ensuremath{\cumthresh^{*}}\xspace}

\newcommand*{\algoCummThresh}{\textsc{\algo-CT}\xspace}
\newcommand*{\algoPeriod}{\textsc{\algo-P}\xspace}
\newcommand*{\period}{\ensuremath{\phi}\xspace}
\newcommand*{\periodopt}{\ensuremath{\period^{*}}\xspace}
\newcommand*{\offset}{\ensuremath{a}\xspace}
\newcommand*{\offsetopt}{\ensuremath{\offset^{*}}\xspace}


%baselines
\newcommand*{\adwin}{\textsc{ADWIN}\xspace}
\newcommand*{\ddm}{\textsc{DDM}\xspace}

%metrics 
\newcommand*{\scpe}{\texttt{SCPE}\xspace}
%datasets
\newcommand*{\covcon}{\textsc{CovCon}\xspace}
\newcommand*{\covconData}{\textsc{\covcon-D}\xspace}
\newcommand*{\covconStatic}{\textsc{\covcon-S}\xspace}
\newcommand*{\Circle}{\textsc{Circle}\xspace}
\newcommand*{\Circles}{\Circle}
\newcommand*{\circles}{\Circle}
\newcommand*{\circlesData}{\textsc{\Circle-D}\xspace}
\newcommand*{\circlesStatic}{\textsc{\Circle-S}\xspace}
\newcommand*{\gauss}{\textsc{Gauss}\xspace}
\newcommand*{\gaussData}{\textsc{\gauss-D}\xspace}
\newcommand*{\gaussStatic}{\textsc{\gauss-S}\xspace}
\newcommand*{\elec}{\textsc{Electricity}\xspace}
\newcommand*{\covertype}{\textsc{Covertype}\xspace}
\newcommand*{\covtype}{\textsc{Covtype}\xspace}
\newcommand*{\airlines}{\textsc{Airlines}\xspace}
\newcommand*{\fixedretraincost}{\ensuremath{46}}


==> tables/real_world_small.tex <==
\begin{tabular}{lccc}
\toprule
Dataset &  \textsc{Cara-T} &  \textsc{Cara-CT} &  \textsc{Cara-P} \\
\midrule
\textsc{Electricity} &             8.32 &             40.32 &            64.07 \\
\textsc{Airlines}    &             6.11 &              5.48 &             5.45 \\
\textsc{Covertype}   &            26.39 &             27.92 &            38.37 \\
\bottomrule
\end{tabular}


==> tables/real_world_small_num_retrains.tex <==
\begin{tabular}{lrrr}
\toprule
Dataset &  \textsc{Cara-T} &  \textsc{Oracle} &  \textsc{ADWIN} \\
                     &                  &                  &                 \\
\midrule
\textsc{Electricity} &             2.39 &             2.36 &            20.0 \\
\textsc{Airlines}    &            27.69 &            25.23 &            24.0 \\
\textsc{Covertype}   &            16.62 &            19.42 &            43.2 \\
\bottomrule
\end{tabular}


==> tables/real_world_small_query_acc.tex <==
\begin{tabular}{lccc}
\toprule
Dataset &  \textsc{Cara-T} &  \textsc{Oracle} &  \textsc{ADWIN} \\
\midrule
\textsc{Electricity} &             0.68 &             0.71 &            0.72 \\
\textsc{Airlines}    &              0.6 &             0.62 &            0.62 \\
\textsc{Covertype}   &             0.66 &             0.76 &             0.8 \\
\bottomrule
\end{tabular}


==> tables/synthetic_small.tex <==
\begin{tabular}{lccc}
\toprule
Dataset &  \textsc{Cara-T} &  \textsc{Cara-CT} &  \textsc{Cara-P} \\
\midrule
\textsc{CovCon-D} &            $17.72$ &             19.26 &             16.3 \\
\textsc{CovCon-S} &            15.58 &             22.94 &           104.79 \\
\midrule
\textsc{Circle-D} &            45.61 &             47.29 &            84.96 \\
\textsc{Circle-S} &            33.89 &             45.15 &            79.34 \\
\midrule
\textsc{Gauss-D}  &             8.63 &             59.93 &           135.95 \\
\textsc{Gauss-S}  &            66.62 &             96.38 &           202.09 \\
\bottomrule
\end{tabular}


==> tables/synthetic_small_num_retrains.tex <==
\begin{tabular}{lrrr}
\toprule
Dataset &  \textsc{Cara-T} &  \textsc{Oracle} &  \textsc{ADWIN} \\
                  &                  &                  &                 \\
\midrule
\textsc{CovCon-D} &            13.89 &             11.2 &            44.8 \\
\textsc{CovCon-S} &            10.05 &             8.21 &            44.8 \\
\textsc{Circle-D} &             5.67 &             3.89 &            11.0 \\
\textsc{Circle-S} &             3.56 &             3.09 &            11.0 \\
\textsc{Gauss-D}  &             2.62 &             2.23 &            31.8 \\
\textsc{Gauss-S}  &             2.57 &             1.92 &            31.8 \\
\bottomrule
\end{tabular}


==> tables/synthetic_small_query_acc.tex <==
\begin{tabular}{lccc}
\toprule
Dataset &  \textsc{Cara-T} &  \textsc{Oracle} &  \textsc{ADWIN} \\
\midrule
\textsc{CovCon-D} &              0.7 &             0.76 &            0.76 \\
\textsc{CovCon-S} &             0.79 &              0.8 &            0.85 \\
\midrule
\textsc{Circle-D} &             0.96 &             0.97 &            0.97 \\
\textsc{Circle-S} &             0.93 &             0.96 &            0.95 \\
\midrule
\textsc{Gauss-D}  &              0.9 &             0.92 &            0.88 \\
\textsc{Gauss-S}  &             0.99 &              1.0 &            0.93 \\
\bottomrule
\end{tabular}


==> tables_LR_SGD/real_world_small.tex <==
\begin{tabular}{lrrr}
\toprule
Dataset &  \textsc{Cara-T} &  \textsc{Cara-CT} &  \textsc{Cara-P} \\
                     &                  &                   &                  \\
\midrule
\textsc{Electricity} &           1031.5 &           1830.55 &          6310.27 \\
\textsc{Airlines}    &            11.68 &             35.89 &            31.38 \\
\textsc{Covertype}   &            28.65 &             35.69 &            40.93 \\
\bottomrule
\end{tabular}


==> tables_LR_SGD/real_world_small_num_retrains.tex <==
\begin{tabular}{lrrr}
\toprule
Dataset &  \textsc{Cara-T} &  \textsc{Oracle} &  \textsc{ADWIN} \\
                     &                  &                  &                 \\
\midrule
\textsc{Electricity} &            18.48 &            13.57 &            13.2 \\
\textsc{Airlines}    &             6.52 &             5.51 &            29.4 \\
\textsc{Covertype}   &             12.2 &             9.29 &            43.6 \\
\bottomrule
\end{tabular}


==> tables_LR_SGD/real_world_small_query_acc.tex <==
\begin{tabular}{lrrr}
\toprule
Dataset &  \textsc{Cara-T} &  \textsc{Oracle} &  \textsc{ADWIN} \\
                     &                  &                  &                 \\
\midrule
\textsc{Electricity} &             0.67 &              0.7 &            0.65 \\
\textsc{Airlines}    &             0.56 &             0.57 &            0.59 \\
\textsc{Covertype}   &             0.63 &             0.72 &            0.75 \\
\bottomrule
\end{tabular}


==> tables_LR_SGD/synthetic_small.tex <==
\begin{tabular}{lrrr}
\toprule
Dataset &  \textsc{Cara-T} &  \textsc{Cara-CT} &  \textsc{Cara-P} \\
                  &                  &                   &                  \\
\midrule
\textsc{CovCon-D} &            27.03 &             16.46 &            13.12 \\
\textsc{CovCon-S} &            55.61 &            126.68 &           449.28 \\
\textsc{Circle-D} &           840.88 &           1067.78 &          1170.57 \\
\textsc{Circle-S} &          1635.49 &            626.12 &           1577.3 \\
\textsc{Gauss-D}  &           148.57 &             216.2 &           211.52 \\
\textsc{Gauss-S}  &           387.83 &            275.75 &          1398.26 \\
\bottomrule
\end{tabular}


==> tables_LR_SGD/synthetic_small_num_retrains.tex <==
\begin{tabular}{lrrr}
\toprule
Dataset &  \textsc{Cara-T} &  \textsc{Oracle} &  \textsc{ADWIN} \\
                  &                  &                  &                 \\
\midrule
\textsc{CovCon-D} &            11.71 &            10.55 &            46.0 \\
\textsc{CovCon-S} &             7.82 &             4.37 &            46.0 \\
\textsc{Circle-D} &             2.32 &             3.23 &             6.8 \\
\textsc{Circle-S} &             0.56 &             2.56 &             6.8 \\
\textsc{Gauss-D}  &             4.72 &             1.32 &            28.2 \\
\textsc{Gauss-S}  &             0.85 &             1.16 &            28.2 \\
\bottomrule
\end{tabular}


==> tables_LR_SGD/synthetic_small_query_acc.tex <==
\begin{tabular}{lrrr}
\toprule
Dataset &  \textsc{Cara-T} &  \textsc{Oracle} &  \textsc{ADWIN} \\
                  &                  &                  &                 \\
\midrule
\textsc{CovCon-D} &             0.66 &             0.77 &            0.74 \\
\textsc{CovCon-S} &             0.67 &             0.62 &            0.91 \\
\textsc{Circle-D} &             0.81 &             0.77 &            0.81 \\
\textsc{Circle-S} &             0.09 &             0.09 &            0.09 \\
\textsc{Gauss-D}  &             0.85 &              0.9 &            0.84 \\
\textsc{Gauss-S}  &              1.0 &              1.0 &             0.7 \\
\bottomrule
\end{tabular}

